Free-Lunch Augmentation by Revisiting Diffusion-Based Data Generation for Cross-Domain Few-Shot Object Detection

Cross-Domain Few-Shot Object Detection (CDFSOD) aims to transfer knowledge from data-rich upstream generic domains to downstream expert domains using scarce training data, where the significant domain gap and data scarcity make it an unsolved challenge. To address this problem, we revisit a natural yet underexplored approach in CDFSOD: data augmentation, by directly synthesizing data through diffusion models to supplement limited training samples. However, due to large domain gaps, we find that current diffusion methods cannot produce good results, leading to performance even lower than using the original images. To address these limitations, we divide the domain gaps into visual gaps and semantic gaps for separate analysis. For the visual gap, we find that the diffusion model cannot distinguish noise from useful information on expert domains, which can be mitigated by adding weakened noise. For the semantic gap, we find that the background semantics shows much smaller gaps between domains than foreground semantics, and we can bridge this gap by background inpainting. Based on the above analysis, we propose a method (Selective Inpainting with Tailored Noise, SITN) to dynamically take different strategies for downstream data synthesis based on their different gaps from the general domain, including a Generation Module for adding tailored noise and a Selection Module to dynamically select the inpainting regions. Extensive experiments on 6 datasets of CDFSOD and 4 datasets of cross-domain few-shot segmentation (CDFSS) validate that we can synthesize helpful data, achieving new state-of-the-art performance. Our codes is available at https://github.com/zzzzj311-droid/Free-Lunch-SITN

==> ______.tex <==
Cross-domain few-shot object detection involves transferring knowledge learned from a source domain to a target domain characterized by scarce samples and significant domain shifts, aiming to achieve rapid detection of objects in the target domain. Due to the dual challenges of data scarcity and domain discrepancy, existing object detection methods based on the source domain often struggle to generalize to the target domain. Focusing on the issue of data scarcity, this study revisits a straightforward yet underexplored approach in cross-domain few-shot object detection: data augmentation—specifically, directly synthesizing data using diffusion models. However, diffusion models cannot be directly adapted to generation tasks, primarily facing two challenges: domain discrepancy and a lack of diversity in foreground object localization.

To address the domain discrepancy between the source and target domains, images generated by diffusion models trained on source domain data exhibit significant distributional differences from target domain images. This study attributes this to the visual differences in style between the source and target domains, as well as the semantic differences between source and target categories, making it difficult for diffusion models to adapt to the target domain. To this end, this study proposes a cross-domain few-shot object detection method based on customized diffusion noise restoration. By adding customized noise, the visual discrepancy is alleviated, and by employing background restoration, the foreground semantic discrepancy is circumvented. Experimental results validate the effectiveness of this method, achieving an average performance improvement of 0.8%–7% across multiple baseline models in cross-domain few-shot object detection tasks.

To address the lack of diversity in foreground object localization, the scarcity of target domain data results in significant variation in the distribution of foreground object sizes within the target dataset, with a particularly acute shortage of small object data. This hampers the ability of object detection models to effectively learn the characteristics of small objects in the target domain. Therefore, this study proposes a cross-domain few-shot object detection method based on diversified diffusion adaptive restoration. Under the premise of alleviating visual discrepancies and circumventing semantic differences, this method generates images with diverse foreground objects. Experimental results show that this method improves the average performance of multiple baseline models in cross-domain few-shot object detection by 2.6%–13%.

In summary, generating target domain data by both mitigating domain discrepancy and enhancing foreground diversity improves the model's generalization capability and adaptation effectiveness in cross-domain few-shot object detection tasks, offering a new research direction for addressing the challenges of domain shift and sample scarcity in object detection.

==> name.tex <==
Cross-domain few-shot object detection (CDFSOD) aims to leverage scarce training data to transfer knowledge from data-rich upstream general domains to downstream specialized domains. This task faces significant domain discrepancies, data scarcity, and inherent issues in object detection models, making it an unresolved challenge. To address this issue, this study revisits a natural yet underexplored approach in cross-domain few-shot object detection: data augmentation—specifically, directly synthesizing data through diffusion models to supplement limited training samples.
However, due to substantial domain discrepancies, existing diffusion methods struggle to achieve desirable results, sometimes even leading to detection performance inferior to using original images. To overcome these limitations, this study decomposes domain discrepancies into visual differences and semantic differences, analyzing them separately, and breaks down the inherent issues in object detection models into performance disparities in detecting small, medium, and large objects.
For visual differences, this study finds that diffusion models cannot distinguish between noise and valid information in the specialized domain, and this issue can be mitigated by incorporating noise weakening. For semantic differences, this study observes that background semantic differences across domains are far smaller than foreground semantic differences, and these can be reduced through background inpainting. Based on these analyses, this study proposes a diffusion-based custom noise selective inpainting method, which dynamically adopts different strategies for data synthesis based on the varying discrepancies between downstream data and the general domain.
Regarding the inherent issues in object detection models, this study identifies that existing object detection models lack proficiency in detecting medium and large objects in cross-domain data, with the problem being particularly severe for small object detection. To address this, this study proposes a diffusion-based diverse adaptive generation method, which achieves the generation of diverse object data by enlarging or reducing the proportion of the foreground in the original image, and designs a filtering mechanism to screen out images that could impair model performance.
This study conducts extensive experiments on six cross-domain few-shot object detection datasets and four cross-domain few-shot segmentation (CDFSS) datasets, with results validating that the proposed method can synthesize effective data and achieve new state-of-the-art performance. In summary, the data augmentation method proposed in this study pushes the performance of cross-domain few-shot object detection to new heights, providing not only a novel systematic data augmentation solution for the issue of data scarcity in cross-domain scenarios but also offering new insights for addressing inherent challenges within the field of object detection.
